Guide the Learner: Controlling Product of Experts Debiasing Method Based on Token Attribution Similarities

Several proposals have been put forward in recent years for improving out-of-distribution (OOD) performance through mitigating dataset biases. A popular workaround is to train a robust model by re-weighting training examples based on a secondary biased model. Here, the underlying assumption is that the biased model resorts to shortcut features. Hence, those training examples that are correctly predicted by the biased model are flagged as being biased and are down-weighted during the training of the main model. However, assessing the importance of an instance merely based on the predictions of the biased model may be too naive. It is possible that the prediction of the main model can be derived from another decision-making process that is distinct from the behavior of the biased model. To circumvent this, we introduce a fine-tuning strategy that incorporates the similarity between the main and biased model attribution scores in a Product of Experts (PoE) loss function to further improve OOD performance. With experiments conducted on natural language inference and fact verification benchmarks, we show that our method improves OOD results while maintaining in-distribution (ID) performance.

==> figs/loss_fig.tex <==
% \begin{figure*}[t!]
% \centering
%     \subfloat{
%         % left bottom right top
%         \includegraphics[width=0.327\textwidth, trim=0 0 0 0, clip] 
%         {./figs/files/Corr_3.pdf}
%     }
%     \subfloat{
%         \includegraphics[width=0.327\textwidth, trim=0 0 0 0, clip] {./figs/files/Uncertain_3.pdf}
%     }
%     \subfloat{
%         \includegraphics[width=0.33\textwidth, trim=0 0 0 0, clip] {./figs/files/Incorr_3.pdf}
%     }
%     \caption{
%     A visualization of our proposed loss function ($\mathcal{L}_{\text{PoE+Sals}}$) based on the biased model's prediction ($f_B^{y_i}(\boldsymbol{x_i})$) and the inter-model similarity ($\rho$).\footnote{We simplify the plots by assuming the output logits of all classes except the gold label are zero for both models ($f_{B/M}^{y\neq y_i}(\boldsymbol{x_i})=0$).}
%     For a given input, when the biased model is correct and certain, the loss will be upweighted when it differs from the main model in terms of saliency scores. However if the biased model returns a certain but incorrect prediction, the loss is downweighted if the main model is dissimilar and also returns a correct prediction. In an uncertain case, the biased model doesn't affect the PoE loss \citr{sanh2020learning}. In this case, the loss is converted to a CE loss based on the output of the main model.
%     }
%     \label{fig:poe_sals_fig_main}
% \end{figure*}
